$\pi$BO: Augmenting Acquisition Functions with User Beliefs for Bayesian Optimization

Bayesian optimization (BO) has become an established framework and popular tool for hyperparameter optimization (HPO) of machine learning (ML) algorithms. While known for its sample-efficiency, vanilla BO can not utilize readily available prior beliefs the practitioner has on the potential location of the optimum. Thus, BO disregards a valuable source of information, reducing its appeal to ML practitioners. To address this issue, we propose $\pi$BO, an acquisition function generalization which incorporates prior beliefs about the location of the optimum in the form of a probability distribution, provided by the user. In contrast to previous approaches, $\pi$BO is conceptually simple and can easily be integrated with existing libraries and many acquisition functions. We provide regret bounds when $\pi$BO is applied to the common Expected Improvement acquisition function and prove convergence at regular rates independently of the prior. Further, our experiments show that $\pi$BO outperforms competing approaches across a wide suite of benchmarks and prior characteristics. We also demonstrate that $\pi$BO improves on the state-of-the-art performance for a popular deep learning task, with a 12.5 $\times$ time-to-accuracy speedup over prominent BO approaches.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> proof.tex <==

\section{Theoretical Analysis} \label{sec:theory_full}
% Kernel of the matern class with smoothness \nu
We now study the \method method from a theoretical standpoint when paired with the EI acquisition function. 
To provide convergence rates, we rely on the set of assumptions introduced by Bull \cite{JMLR:v12:bull11a}. 
These assumptions are satisfied for popular kernels like the Matérn~\cite{matern1960spatial} class and the Gaussian kernel, which is obtained in the limit $\nu \rightarrow \infty$, 
where the rate $\nu$ controls the smoothness of functions from the GP prior.
Our theoretical results apply when both length scales ${\bm{\ell}}$ and the global scale of variation $\sigma$ are fixed; these results can then be extended to the case where the kernel hyperparameters are learned using Maximum Likelihood Estimation (MLE) following the same procedure as in Bull \cite{JMLR:v12:bull11a} (Theorem 5).
We define the loss over the ball $B_R$ for a function $f$ of norm $||f||_{\mathcal{H}_{\bm{\ell}}(\mathcal{X})} \leq R$ in the RKHS $\mathcal{H}_{\bm{\ell}}(\mathcal{X})$ given a symmetric positive-definite kernel $K_{\bm{\ell}}$ as
\begin{equation} \label{eq:loss}
    \mathcal{L}_{n}(u, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R) \overset{\Delta}{=} \sup_{{||f||}_{\mathcal{H}_{\bm{\ell}}(\mathcal{X})}\leq R}\mathbb{E}^u_f[f(\bm{x}^*_n) - \min f],
\end{equation}
where $n$ is the optimization iteration and $u$ a strategy.
We focus on the strategy that maximizes \pei{} and show that the loss in \eqref{eq:loss} can, at any iteration $n$, be bounded by the vanilla EI loss function. 
We refer to $\text{EI}_{\pri, n}$ and $\text{EI}_{n}$ when we want to emphasize the iteration $n$ for the acquisition functions $\text{EI}_{\pri}$ and $\text{EI}$, respectively. 
\begin{theorem} \label{th1}
Given $\mathcal{D}_n$, $K_{\bm{\ell}}$, $\pri$, $\sigma$, ${\bm{\ell}}$, $R$ and the compact set $\mathcal{X}\subset\mathbb{R}^d$ as defined above, the loss $\mathcal{L}_{n}$ incurred at iteration $n$ by $\text{EI}_{\pri, n}$
%when considering the next design point $\bm{x}_{n+1}$ 
% Given (everything mentioned above) this, this and this that as defined above,  - BR is ball, n is iteration in BO
can be bounded from above:
%by the loss incurred by vanilla EI, multiplied by a factor that tends to 1 as $n\rightarrow \infty$:
\begin{equation}
    \mathcal{L}_{n}(\text{EI}_{\pri, n}, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R) \leq C_{\pi, n} \mathcal{L}_{n}(\text{EI}_n, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R), \quad C_{\pi, n} = \left(\frac{\max_{\xinx} \pi(\bm{x})}{\min_{\xinx} \pi(\bm{x})}\right)^{\beta/n}.
\end{equation}
\end{theorem}  

\begin{proof}
To bound the performance of \pei{} to that of EI, we primarily need to consider Lemma~7 and Lemma~8 by Bull \cite{JMLR:v12:bull11a}. In Lemma~7, it is stated that for any sequence of points $\{\bm{x}_i\}_{i=1}^n$, $p \in \mathbb{N}$ 
and kernel length scales ${\bm{\ell}}$, the posterior variance $s^2_n$ 
on $\bm{x}_{n+1}$ will satisfy the following inequality at most $p$ times, with $p < n$, 
%can be bounded in the number of times $p$ that the variance exceeds a large value as
\begin{equation} \label{varbound}
    s_n(\bm{x}_{n+1}; \bm{\ell}) \geq Cp^{-(\nu \land 1)/d}(\log p)^\gamma), \quad \gamma = \begin{cases}
		\alpha, & \nu \leq 1\\
        0, & \nu > 1
	\end{cases}
\end{equation}
%In other words, Lemma~7 says that \eqref{varbound} can only happen for $p$ of the $n$ total $x_i$. 
Thus, we can bound the posterior variance by assuming a point in time $n_p$ where Eq. \ref{varbound} has held $p$ times. 
We now consider Lemma 8 where, through a number of inequalities, EI is bounded by the actual improvement $I_n$
\begin{equation}
    \max\left(I_n-Rs, \frac{\tau(-R/\sigma)}{\tau(R/\sigma)}I_n   \right) \leq \eixn \leq I_n + (R + \sigma)s,
\end{equation}
where $I_n = (f(\bm{x}^*_n) - f(\bm{x}))^+$, $\tau(z) = z\Phi(z) + \phi(z)$ and $s = s_n(\bm{x}_{n}; \bm{\ell})$. Since \method reweights $\text{EI}_n$ by $\pri_n$, these bounds need adjustment to hold for $\text{EI}_{\pi, n}$. 
For the upper bound provided in Lemma~8, we make use of $\max_{\xinx} \pri_n(\bm{x})$ to bound $\peixn$ %to $\eixn$ 
for any point $\xinx$: 
\begin{equation}
    \frac{\peixn} {\max_{\xinx} \pri_n(\bm{x})} = \frac{\eixn \pri_n(\bm{x})} {\max_{\xinx}\pri_n(\bm{x})} \leq \eixn \leq I_n + (R + \sigma)s.
\end{equation}
For the lower bounds, we instead rely on $\min_{\xinx} \pri_n(\bm{x})$ in a similar manner:
\begin{equation}
    \max\left(I_n-Rs, \frac{\tau(-R/\sigma)}{\tau(R/\sigma)}I_n   \right) \leq \eixn \leq \frac{\eixn \pri_n(\bm{x})} {\min_{\xinx}\pri_n(\bm{x})}  = \frac{\peixn} {\min_{\xinx} \pri_n(\bm{x})}.
\end{equation}
Consequently, \pei{} can be bounded by the actual improvement as
\begin{equation}
    {\min_{\xinx}\pri_n(\bm{x})}\max\left(I_n-Rs, \frac{\tau(-R/\sigma)}{\tau(R/\sigma)}I_n\right) \leq \peixn \leq {\max_{\xinx}\pri_n(\bm{x})} (I_n + (R + \sigma)s). 
\end{equation}
With these bounds in place, we consider the setting as in the proof for Theorem 2 in Bull \cite{JMLR:v12:bull11a}, which proves an upper bound for the EI strategy in the fixed kernel parameters setting. 
At an iteration $n_p, p \leq n_p \leq 3p$, the posterior variance will be bounded by $Cp^{-(\nu \land 1)/d}(\log p)^\gamma$. Furthermore, since $I_n \geq 0$ and $||f||_{\mathcal{H}_\ell(\mathcal{X}))} \leq R$, we can bound the total improvement as
\begin{equation}
    \sum_i I_i \leq \sum_i f(\bm{x}^*_{i}) - f(\bm{x}^*_{i+1}) \leq f(\bm{x}^*_1) - \min f \leq 2||f||_\infty \leq 2R,
\end{equation}
leaving us a maximum of $p$ times that $I_n \geq 2Rp^{-1}$. Consequently, both the posterior variance $s^2_{n_p}$ and the improvement $I_{n_p}$ are bounded at $n_p$. For a future iteration $n,\; 3p \leq n \leq 3(p+1)$, we use the  bounds on \pei, $s_{n_p}$ and $I_{n_p}$ to obtain the bounds on the loss on \pei{}:
\begin{equation} \label{eq:bound_loss}
\begin{split}
    &\mathcal{L}_{n}(\text{EI}_\pri, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R) \\
    &= f(\bm{x}_n^*) - \min f \\
    &\leq  f(\bm{x}_{n_p}^*) - \min f \\
    &\leq\frac{\text{EI}_{\pi,n_p}(\bm{x}^*)}{\min_{\xinx}\pri_n(\bm{x})}  \frac{\tau (R/\sigma)}{\tau (-R/\sigma)} \\
    &\leq
    \frac{\text{EI}_{\pi,n_p}(\bm{x}_{n+1})}{\min_{\xinx}\pri_n(\bm{x})}  \frac{\tau (R/\sigma)}{\tau (-R/\sigma)} \\
    &\leq\frac{\min_{\xinx}\pri_n(\bm{x})}{\min_{\xinx}\pri_n(\bm{x})}  \frac{\tau (R/\sigma)}{\tau (-R/\sigma)}
    \left(I_{n_p} + (R+\sigma)s_{n_p}\right)\\
    &\leq\left(\frac{\max_{\xinx}\pri(\bm{x})}{\min_{\xinx}\pri(\bm{x})}\right)^{\beta/n}  \frac{\tau (R/\sigma)}{\tau (-R/\sigma)} (2Rp^{-1} + (R+\sigma)Cp^{-(\nu \land 1)/d}(\log p)^\gamma),
\end{split}
\end{equation}
where the last inequality in Eq. \ref{eq:bound_loss} is a factor $C_{\pri, n} = \left(\frac{\max_{\xinx}\pri(\bm{x})}{\min_{\xinx}\pri(\bm{x})}\right)^{\beta/n}$ larger than the bound on $\mathcal{L}_n(\text{EI}, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R)$.
\end{proof} 
\begin{corollary} The loss of a decaying prior-weighted Expected Improvement strategy, \pei, is asymptotically equal to the loss of an Expected Improvement strategy, EI:
\begin{equation}
    \mathcal{L}_{n}(\text{EI}_\pri, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R) \sim  \mathcal{L}_{n}(\text{EI}, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R),
\end{equation}

so we obtain a convergence rate for \pei{} of $\mathcal{L}_{n}(\text{EI}_\pri, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R) = \mathcal{O}(n^{-(\nu \land 1)/d}(\log n)^\gamma)$.
\end{corollary}
\begin{proof}
For Corollary 1, we simply compute the fraction of the losses in the limit,
\begin{equation}
    \lim_{n \to \infty}\frac{\mathcal{L}_n(\text{EI}_\pi, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R)}{\mathcal{L}_n(\text{EI}, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R)} \le \lim_{n \to \infty} \left(\frac{\max_{\xinx}\pri(\bm{x})}{\min_{\xinx}\pri(\bm{x})}\right)^{\beta/n} =1.
\end{equation}
\end{proof}
Thus, we determine that weighting introduced by \pei{} does not negatively impact the worst-case convergence rate. The short-term performance is controlled by the user in their choice of $\pri(\bm{x})$ and $\beta$. This result is coherent with intuition, as a weaker prior or quicker decay will yield a short-term performance closer to that of EI. On the contrary, a stronger prior or slower decay is not guaranteed the same short-term performance, but can produce better empirical results, as shown in our experiments in Section~\ref{results}.


==> proofsketch.tex <==
\subsection{Theoretical Analysis} \label{sec:theory}
% Kernel of the matern class with smoothness \nu
We now study the \method method from a theoretical standpoint when paired with the EI acquisition function. 
To provide convergence rates, we rely on the set of assumptions introduced by Bull \citep{JMLR:v12:bull11a}. 
These assumptions are satisfied for popular kernels like the Matérn~\citep{matern1960spatial} class and the Gaussian kernel, which is obtained in the limit $\nu \rightarrow \infty$, 
where the rate $\nu$ controls the smoothness of functions from the GP prior.
Our theoretical results apply when both length scales ${\bm{\ell}}$ and the global scale of variation $\sigma$ are fixed; these results can then be extended to the case where the kernel hyperparameters are learned using Maximum Likelihood Estimation (MLE) following the same procedure as in Bull \citep{JMLR:v12:bull11a} (Theorem 5).
%\frank{Could we say: ``We detail this extension in Appendix X.'', or is this going to be complicated?}
We define the loss over the ball $B_R$ for a function $f$ of norm $||f||_{\mathcal{H}_{\bm{\ell}}(\mathcal{X})} \leq R$ in the RKHS $\mathcal{H}_{\bm{\ell}}(\mathcal{X})$ given a symmetric positive-definite kernel $K_{\bm{\ell}}$ as
\begin{equation} \label{eq:loss_mainpaper}
    \mathcal{L}_{n}(u, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R) \overset{\Delta}{=} \sup_{{||f||}_{\mathcal{H}_{\bm{\ell}}(\mathcal{X})}\leq R}\mathbb{E}^u_f[f(\bm{x}^*_n) - \min f],
\end{equation}
where $n$ is the optimization iteration and $u$ a strategy. We focus on the strategy that maximizes the prior-weighted EI, \pei{}, and show that the loss in \eqref{eq:loss_mainpaper} 
%\frank{Eq. (23) is probably in the appendix. Should this refere to Eq. (7)?}
can, at any iteration $n$, be bounded by the vanilla EI loss function. 
We refer to $\text{EI}_{\pri, n}$ and $\text{EI}_{n}$ when we want to emphasize the iteration $n$ for the acquisition functions $\text{EI}_{\pri}$ and $\text{EI}$, respectively. 

%PROOF SKETCH
\begin{theorem} \label{th1}
Given $\mathcal{D}_n$, $K_{\bm{\ell}}$, $\pri$, $\sigma$, ${\bm{\ell}}$, $R$ and the compact set $\mathcal{X}\subset\mathbb{R}^d$ as defined above, the loss $\mathcal{L}_{n}$ incurred at iteration $n$ by $\text{EI}_{\pri, n}$
can be bounded from above as
%Given $\mathcal{D}_n$, $K_{\bm{\ell}}$, $\pri$, $\sigma$, ${\bm{\ell}}$ and R, the loss $\mathcal{L}_{n}$ incurred at iteration $n$ by $\text{EI}_{\pri, n}$
%%when considering the next design point $\bm{x}_{n+1}$ 
% Given (everything metioned above) this, this and this that as defined above,  - BR is ball, n is iteration in BO
%can be bounded from above as:
%by the loss incurred by vanilla EI, multiplied by a factor that tends to 1 as $n\rightarrow \infty$:
\begin{equation}
    \mathcal{L}_{n}(\text{EI}_{\pri, n}, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R) \leq C_{\pi, n} \mathcal{L}_{n}(\text{EI}_n, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R), \quad C_{\pi, n} = \left(\frac{\max_{\xinx} \pi(\bm{x})}{\min_{\xinx} \pi(\bm{x})}\right)^{\beta/n}.
\end{equation}
\end{theorem}  
\textit{Proof sketch (for the full proof, see Appendix \ref{sec:appendix_proof}):} 
To bound the performance of \pei{} to that of EI, we need to establish three bounds: an upper bound on the posterior variance $s_n^2$, and a lower and upper bound on \pei{} in relation to the actual improvement  $I_n$ at iteration $n$. 

\textbf{Upper Bound on Variance}\quad
Lemma 7 in Bull~\citep{JMLR:v12:bull11a} provides an upper bound on the variance that depends on $\mathcal{X}$,$K_{\bm{\ell}}$, $\sigma$ and ${\bm{\ell}}$, but not on the strategy $u$. Specifically, for any sequence of points $\{\bm{x}_i\}_{i=1}^n$, $p \in \mathbb{N}$, the posterior variance $s^2_n$ 
will be ``large'' at most $p$ times, which holds for any $p\in \mathbb{N}$. 
%\frank{I don't fully understand the previous sentence. Should we put ``large'' in quotes, as we cannot fully define it here?}
Thus, the required bound on the variance is unaffected by choosing \pei{} as our strategy.
%\carl{this requires quite a bit to properly specify, so I just went with large - I guess we can hgo with quotes.}

\textbf{Improvement-related Bounds}\quad
Lemma 8 in Bull~\citep{JMLR:v12:bull11a} bounds EI by the actual improvement $I$ as
\begin{equation}
    \max\left(I_n-Rs, \frac{\tau(-R/\sigma)}{\tau(R/\sigma)}I_n   \right) \leq \eixn \leq I_n + (R + \sigma)s.
\end{equation}
Moreover, we can bound \pei{} to EI accordingly:
\begin{equation}
    {\min_{\xinx}\pri_n(\bm{x})}\eixn \leq \peixn \leq {\max_{\xinx}\pri_n(\bm{x})}\eixn.
\end{equation}
Combining these bounds yields a bound on \pei{} to $I$ as
\begin{equation} \label{eq:newbound}
    {\min_{\xinx}\pri_n(\bm{x})}\max\left(I_n-Rs, \frac{\tau(-R/\sigma)}{\tau(R/\sigma)}I_n\right) \leq \peixn \leq {\max_{\xinx}\pri_n(\bm{x})} (I_n + (R + \sigma)s), 
\end{equation}
which gives us an improvement-related bound wider than that of EI, but converging towards it for a decaying prior. With these bounds in place, we consider an iteration $n_p$ when $I_{n_p}$ and $s_{n_p}$ are both upper bounded, and use the inequality in \eqref{eq:newbound}. Then, for all future iterations $n$, we obtain the factor $C_{n, \pri}$ governing the loss $\mathcal{L}_{n}(\text{EI}_\pri, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R)$ relative $\mathcal{L}_{n}(\text{EI}, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R)$. \hfill$\square$ 
%\frank{Is the last line a typo? The second-last term and the last term appear to be identical?}

Using Theorem \ref{th1}, we can obtain the convergence rate of \pei{}. This trivially follows 
%from the theorem 
when considering the fraction of the losses in the limit and inserting the original convergence rate on EI provided in Bull~\citep{JMLR:v12:bull11a}:

\begin{corollary} The loss of a decaying prior-weighted Expected Improvement strategy, \pei{}, is asymptotically equal to the loss of an Expected Improvement strategy, EI:
\begin{equation}
    \mathcal{L}_{n}(\text{EI}_{\pri, n}, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R) \sim  \mathcal{L}_{n}(\text{EI}_n, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R),
\end{equation}

so we obtain a convergence rate for \pei{} of $\mathcal{L}_{n}(\text{EI}_{\pri, n}, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R) = \mathcal{O}(n^{-(\nu \land 1)/d}(\log n)^\gamma)$.
\end{corollary}

Thus, we determine that the weighting introduced by \pei{} does not negatively impact the worst-case convergence rate. The short-term performance is controlled by the user in their choice of $\pri(\bm{x})$ and $\beta$. This result is coherent with intuition, as a weaker prior or quicker decay will yield a short-term performance closer to that of EI. On the contrary, a stronger prior or slower decay is not guaranteed the same short-term performance, but can produce better empirical results, as shown in our experiments in Section~\ref{results}.

==> throwaway.tex <==
% Proof sketch
\textit{Proof sketch (for the full proof, see Appendix \ref{sec:appendix_proof}):} 
To bound the performance of \pei{} to that of EI, we need to establish three bounds: an upper bound on the posterior variance $s_n^2$, and a lower and upper bound on \pei{} in relation to the actual improvement  $I_n$ at iteration $n$. 

\textbf{Upper Bound on Variance}\quad
Lemma 7 in \citet{JMLR:v12:bull11a} provides an upper bound on the variance that depends on $\mathcal{X}$,$K_{\bm{\ell}}$, $\sigma$ and ${\bm{\ell}}$, but not on the strategy $u$. Specifically, for any sequence of points $\{\bm{x}_i\}_{i=1}^n$, $p \in \mathbb{N}$, the posterior variance $s^2_n$ 
will be ``large'' at most $p$ times, which holds for any $p\in \mathbb{N}$. 
%\frank{I don't fully understand the previous sentence. Should we put ``large'' in quotes, as we cannot fully define it here?}
Thus, the required bound on the variance is unaffected by choosing \pei{} as our strategy.
%\carl{this requires quite a bit to properly specify, so I just went with large - I guess we can hgo with quotes.}

\textbf{Improvement-related Bounds}\quad
Lemma 8 in \citet{JMLR:v12:bull11a} bounds EI by the actual improvement $I$ as
\begin{equation}
    \max\left(I_n-Rs, \frac{\tau(-R/\sigma)}{\tau(R/\sigma)}I_n   \right) \leq \eixn \leq I_n + (R + \sigma)s.
\end{equation}
Moreover, we can bound \pei{} to EI accordingly:
\begin{equation}
    {\min_{\xinx}\pri_n(\bm{x})}\eixn \leq \peixn \leq {\max_{\xinx}\pri_n(\bm{x})}\eixn.
\end{equation}
Combining these bounds yields a bound on \pei{} to $I$ as
\begin{equation} \label{eq:newbound}
    {\min_{\xinx}\pri_n(\bm{x})}\max\left(I_n-Rs, \frac{\tau(-R/\sigma)}{\tau(R/\sigma)}I_n\right) \leq \peixn \leq {\max_{\xinx}\pri_n(\bm{x})} (I_n + (R + \sigma)s), 
\end{equation}
which gives us an improvement-related bound wider than that of EI, but converging towards it for a decaying prior. With these bounds in place, we consider an iteration $n_p$ when $I_{n_p}$ and $s_{n_p}$ are both upper bounded, and use the inequality in \eqref{eq:newbound}. Then, for all future iterations $n$, we obtain the factor $C_{n, \pri}$ governing the loss $\mathcal{L}_{n}(\text{EI}_\pri, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R)$ relative $\mathcal{L}_{n}(\text{EI}, \mathcal{D}_n, \mathcal{H}_{\bm{\ell}}(\mathcal{X}), R)$. \hfill$\square$ 
%\frank{Is the last line a typo? The second-last term and the last term appear to be identical?}





\section{Limitations} \label{sec:limitations}
 \textbf{Performance Claims and Prior Assessment} \quad
 When assessing approaches relying on user beliefs, priors are naturally required to assess the effectiveness of the approach. Moreover, different prior qualities should be used to address high-end performance as well as robustness. In Section \ref{results}, we construct priors of simple design, to reflect general types of prior quality. However, the quality of a prior is ultimately arbitrary, both in the synthetic and real-world setting. We attempt to alleviate this issue by relying on quantitative methods and default settings chosen by experts for our priors.
 
 \textbf{Dependence on Supporting Framework}\quad
While one of \method's main strengths is its cross-framework flexibility, its performance is also reliant on the effectiveness of that supporting BO framework. This makes \method difficult to evaluate by itself. While \method's theoretical properties makes it fundamentally robust, its empirical performance and benefits from the prior will likely vary between frameworks. 
 
  \textbf{Acquisition Function Restrictions}\quad
We propose the use of \method with a collection of acquisition functions which all select design points through myopic criteria. However, \method should not be used with non-myopic functions, as neither the fundamental purposes nor the selection procedures of these acquisition functions are well-aligned with \method. While we do believe that \method could be extended to this setting, the approach will ultimately have to be modified in order to make this feasible.

\section{Broader Impact} \label{sec:impact}

Our work proposes a novel BO approach that combines users' prior knowledge about the location of the optimum with BO's acquisition function. The approach is foundational and thus will not bring direct societal or ethical consequences. However, \method will likely be used in the development of applications for a wide range of areas and thus indirectly contribute to their impacts on society. In particular, we envision that \method will impact a multitude of fields by allowing ML experts to inject their knowledge about the location of the optimum into BO. We recall that only a small fraction of recent ML research has used BO for hyperparameter tuning, as practitioners have often favored manual tuning~\cite{bouthillier:survey}. \method has the potential to bridge this gap and increase the adoption of BO, helping experts fine-tune solutions faster and better. 

%We envision that our work will have a deep indirect impact in society. For instance, Bayesian Optimization has been used in conjunction with environmental monitoring~\citep{marchant2012bayesian}, which could improve how we protect natural resources and help quickly detect and prevent environmental disasters. Bayesian Optimization has also been used in computer vision~\citep{nardi2017algorithmic}, where it could lead to positive breakthroughs, such as improved medical imaging systems, or controversial developments, such as improved public surveillance. 

We also envision that \method will have an impact in the democratization of ML. Currently, ML models require expert knowledge in order to fine-tune models and achieve good performance in new applications. The effectiveness of BO in AutoML~\cite{feurer_autosklearn, vanschoren2019meta} and hyperparameter tuning~\cite{spearmint, falknerKH18} has already been demonstrated. We believe \method will bolster this impact. Though non-ML experts may not have priors of their own, they still can leverage the priors established by experts through defaults. In the future, we envision that experts might even provide defaults for these priors together with public implementations of their new algorithms. %For instance, they might leverage the public image dataset priors proposed by~\citet{navruzyan19fastai}.

We intend for \method to be a tool that allows users to assist BO by providing reasonable prior knowledge and beliefs. This process induces user bias into the optimization, as \method will inevitably start by optimizing around this prior. As some users may only be interested in optimizing in the direct neighborhood of their prior, \method{} could allow them to do so if provided with a high $\beta$ value in relation to the number of iterations. Thus, if improperly specified, \method could serve to reinforce user's beliefs by providing improved solutions only for the user's region of interest. 

Finally, the demonstrated speedup of \method has the potential of reducing the amount of BO iterations required in order to yield sufficient model performance, assuming prior knowledge is available on the task at hand. As a consequence, model tuning can be done in less time and with less energy usage, making \method a useful tool for reducing carbon emissions related to model training.

%\method impacts not only the performance of applications, but also makes the development of new applications more accessible. By automating design decisions, Bayesian Optimization alleviates the expertise required to design and fine-tune new applications. For instance, Bayesian Optimization can be used for tuning ML hyperparameters, supporting non-ML experts to apply ML in their applications. This is particularly true for \method, which enables users to inject their current experience into the optimization process. For example in Section~\ref{sec:experiments.spatial}, \method combines the expertise of a \spatial developer into Bayesian Optimization to achieve better performance than Bayesian Optimization or the expert had achieved before separated. However, this could also help the development of new malicious applications.

%Our results with \spatial also directly impacts the hardware design field. We show that \method can be directly integrated with \spatial to lead to better specialized hardware designs. For instance, this compounds with \method's impact on ML by also enabling the development of specialized hardware for ML models~\citep{hadjis2019tensorflow}. Likewise, \method and \spatial enable the design of efficient hardware for cybersecurity primitives for the Internet of Things and Cyber-Physical-Systems, where traditional cybersecurity solutions are too expensive and often impractical~\citep{wu2017new}.


%We believe \method has the potential for deep societal impact. In particular, we believe \method will lead to a surge on the number and quality of new applications in a wide range of fields, by automatically optimizing design decisions. As with any other new technology, \method may give rise to both positive and negative new applications. 

%\frank{Optimally, if we have time before submission, it would be good to have consistent references; either all first names written out or not.
%In our group's bibtex file, we only use abbreviated first names (since for some papers full names are not available).}

